Complete CALM: A Unified Criterion for Coordination

Coordination is often the dominant cost in concurrent systems. When is it intrinsically needed? Too little produces heisenbugs; too much adds latency and sacrifices availability. CALM, CAP, and CRDTs each answer the question for one class of programs, consistency models, or design patterns, in formalisms that cannot be compared or combined, which leaves developers guessing. We provide a simple formalism that unifies the literature and offers new results. An I/O Specification (spec) is a possibility table containing, for each input, every output a system may produce, with partial orders on inputs and outputs. Its runs are consistent when they are confluent as input grows. Functional CALM generalizes the CALM Theorem from Datalog to any function between ordered domains: the runs are consistent exactly when the function is monotone. Complete CALM extends this to nondeterministic specs, where the test is Lifted Monotonicity; Complete CAP follows as a corollary. Highly Available Transactions, Invariant Confluence, and later CALM refinements map into the same framework. Prior CALM results stop at monotonicity: for non-monotone specs, they say only that coordination is needed somewhere. Our framework offers constructive results on both sides: it says exactly what coordination a spec needs, and when. A non-monotone spec's outputs drive irrevocable commitments that are required for consistency, enforceable by coordination mechanisms like locks, atomics, or consensus. A composition of specs has tight coordination when the commitments of an upstream stage are necessary and sufficient for later stages. We show how to order the upstream's outputs to achieve it, explaining designs such as consensus logs in front of a replicated store.

==> acmart-preload-hook.tex <==
% Compatibility shim for the CIDR 2027 class (acmart v1.78).
% Current hyperxmp requires hyperref to have been loaded first, while the
% supplied class loads them in the opposite order. The class intentionally
% loads this hook before its packages.
\RequirePackage[bookmarksnumbered,unicode]{hyperref}

